Principal Geodesic Analysis in Director-Based Dynamics of Hybrid Mechanical Systems

In this article, we present new computational realizations of principal geodesic analysis for the unit sphere $S^2$ and the special orthogonal group $SO(3)$. In particular, we address the construction of long-time smooth lifts across branches of the respective logarithm maps. To this end, we pay special attention to certain critical numerical aspects such as singularities and their consequences on the numerical precision. Moreover, we apply principal geodesic analysis to investigate the behavior of several mechanical systems that are very rich in dynamics. The examples chosen are computationally modeled by employing a director-based formulation for rigid and flexible mechanical systems. Such a formulation allows to investigate our algortihms in a direct manner while avoiding the introduction of additional sources of error that are unrelated to principal geodesic analysis. Finally, we test our numerical machinery with the examples and, at the same time, we gain deeper insight into their dynamical beahvior.

==> abbr.tex <==
% Abbreviations -- requires package xspace

\newcommand\abbrfont{}

\newcommand\abbr[1][abbrev]{{\abbrfont{#1.}}\xspace}
\newcommand\abbrev{\abbr}
\providecommand\ca{\abbr[ca]}% Also in abk.tex.
\newcommand\cf{\abbr[cf]}
\newcommand\eg{\abbr[e.g]}
\providecommand\etal{\abbr[et~al]}% Also in abk.tex.
\providecommand\etc{\abbr[etc]}% Also in abk.tex.
\newcommand\ie{\abbr[i.e]}
\newcommand\resp{\abbr[resp]}
\providecommand\vs{\abbr[vs]}% Also in abk.tex.
\newcommand\Wlog{\abbr[w.l.o.g]}% \wlog is an internal logging command.
\newcommand\wrt{\abbr[w.r.t]}


==> code-names.tex <==
% Code names -- requires packages xspace and relsize

\providecommand{\sfnamesize}{\relsize{0}}
\providecommand{\sfname}[1]{\textsf{\sfnamesize#1}\xspace}

\newcommand{\plusplus}{\raisebox{0.15ex}{++}}
\newcommand{\ALADIN}{\sfname{ALADIN}}
\newcommand{\AMPL}{\sfname{AMPL}}
\newcommand{\BARON}{\sfname{BARON}}
\newcommand{\Bash}{\sfname{Bash}}
\newcommand{\BGL}{\sfname{BGL}}
\newcommand{\BLAS}{\sfname{BLAS}}
\newcommand{\Bonmin}{\sfname{Bonmin}}
\newcommand{\boost}{\sfname{boost}}
\newcommand{\Boost}{\sfname{Boost}}
\newcommand{\BoostMPI}{\sfname{Boost.MPI}}
\newcommand{\langC}{\sfname{C}}
\newcommand{\CC}{\sfname{C\plusplus}}
\newcommand{\Cpp}{\CC}
\newcommand{\CCEleven}{\sfname{C\plusplus 11}}
\newcommand{\CppEleven}{\CCEleven}
\newcommand{\CCFourteen}{\sfname{C\plusplus 14}}
\newcommand{\CppFourteen}{\CCFourteen}
\newcommand{\Clean}{\sfname{Clean}}
\newcommand{\clean}{\sfname{clean}}
\newcommand{\CleanIPM}{\sfname{Clean::IPM}}
\newcommand{\cleanIPM}{\sfname{clean::ipm}}
\newcommand{\CONOPT}{\sfname{CONOPT}}
\newcommand{\CONOPTfour}{\sfname{CONOPT4}}
\newcommand{\CPLEX}{\sfname{CPLEX}}
\newcommand{\CUTE}{\sfname{CUTE}}
\newcommand{\CUTEr}{\sfname{CUTEr}}
\newcommand{\CUTEst}{\sfname{CUTEst}}
\newcommand{\dealII}{\sfname{deal.II}}
\newcommand{\DICOPT}{\sfname{DICOPT}}
\newcommand{\DOpElib}{\sfname{DOpElib}}
\newcommand{\DOM}{\sfname{DOM}}
\newcommand{\Doxygen}{\sfname{Doxygen}}
\newcommand{\EPANET}{\sfname{EPANET}}
\newcommand{\Excel}{\sfname{Excel}}
\newcommand{\FilterSQP}{\sfname{FilterSQP}}
\newcommand{\filtermpec}{\sfname{filtermpec}}
\newcommand{\GAMS}{\sfname{GAMS}}
\newcommand{\GasLib}{\sfname{GasLib}}
\newcommand{\GCC}{\sfname{GCC}}
\newcommand{\Gurobi}{\sfname{Gurobi}}
\newcommand{\Fortran}{\sfname{Fortran}}
\newcommand{\FortranSS}{\sfname{Fortran 77}}
\newcommand{\iGNO}{\sfname{iGNO}}
\newcommand{\Ipopt}{\sfname{Ipopt}}
\newcommand{\IPM}{\sfname{IPM}}
\newcommand{\Java}{\sfname{Java}}
\newcommand{\KNITRO}{\sfname{KNITRO}}
\newcommand{\KNITRODIRECT}{\sfname{KNITRO/DIRECT}}
\newcommand{\KNITROCG}{\sfname{KNITRO/CG}}
\newcommand{\LaGO}{\sfname{LaGO}}
\newcommand{\Lamatto}{\sfname{LaMaTTO\plusplus}}
\newcommand{\LAPACK}{\sfname{LAPACK}}
\newcommand{\Liwacom}{\sfname{Liwacom}}
\newcommand{\LOQO}{\sfname{LOQO}}
\newcommand{\MacMPEC}{\sfname{MacMPEC}}
\newcommand{\Matlab}{\sfname{Matlab}}
\newcommand{\MINLPLib}{\sfname{MINLPLib}}
\newcommand{\MINOS}{\sfname{MINOS}}
\newcommand{\MOSEK}{\sfname{MOSEK}}
\newcommand{\MPC}{\sfname{MPC}}
\newcommand{\MPI}{\sfname{MPI}}
\newcommand{\MSIPM}{\sfname{MSIPM}}
\newcommand{\MSKKT}{\sfname{MSKKT}}
\newcommand{\MSSQP}{\sfname{MSSQP}}
\newcommand{\MSTOP}{\sfname{MSTOP}}
\newcommand{\OOPS}{\sfname{OOPS}}
\newcommand{\openMPI}{\sfname{Open MPI}}
\newcommand\Pardiso{\sfname{Pardiso}}
\newcommand{\Python}{\sfname{Python}}
\newcommand{\SCIP}{\sfname{SCIP}}
\newcommand{\Simone}{\sfname{SIMONE}}
\newcommand{\SNOPT}{\sfname{SNOPT}}
\newcommand{\SQP}{\sfname{SQP}}
\newcommand{\TreeKKT}{\sfname{TreeKKT}}
\newcommand{\Xerces}{\sfname{Xerces}}
\newcommand{\XML}{\sfname{XML}}
\newcommand{\Zimpl}{\sfname{Zimpl}}


==> math-fields.tex <==
% Math fields -- requires amsfonts

\newcommand{\field}{\mathbb}

% "natural" names
\newcommand{\complex}{\field{C}}
\newcommand{\quaternions}{\field{H}}
\newcommand{\naturals}{\field{N}}
\newcommand{\polynomials}{\field{P}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}

% alternative names
\newcommand{\numsetC}{\complex}
\newcommand{\numsetH}{\quaternions}
\newcommand{\numsetN}{\naturals}
\newcommand{\numsetQ}{\rationals}
\newcommand{\numsetR}{\reals}
\newcommand{\numsetZ}{\integers}

% short names
\makeatletter
\@ifundefined{C}{\newcommand{\C}{\complex}}
{\PackageInfo{math-fields}{Use \string\field{C} for complex numbers;
 \MessageBreak command \string\C\space already defined}{}}
\makeatother
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}
\newcommand{\Poly}{\polynomials}% deprecated: NuMa scripts


==> math-std.tex <==
% Standard math definitions -- requires amsmath

\providecommand\const{\textup{const}}% Also defined in documentclass siamltex.
\newcommand\qtext{\quad\text}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\ifgiven[3]{\def\fc@rg{#1}\ifx\fc@rg\empty#3\else#2\fi}
\newcommand\fcarg[1]{\ifgiven{#1}\fc@rg\fcdot}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\tfracabs[2]{\abs{#1}/\abs{#2}}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\tabsfrac\tfracabs
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\pcolon{\mathpunct:}
\newcommand\defsep\pcolon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\tfracnorm[3][]{\norm[#1]{#2}/\norm[#1]{#3}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\tnormfrac\tfracnorm
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\tfracnormpow[4][]{\norm[#1]{#2}^{#4}/\norm[#1]{#3}^{#4}}
\newcommand\fracnormpow[4][]{\frac{\norm[#1]{#2}^{#4}}{\norm[#1]{#3}^{#4}}}
\newcommand\fracNormpow[4][]{\frac{\Norm[#1]{#2}^{#4}}{\Norm[#1]{#3}^{#4}}}
\newcommand\pfrac[2]{\frac{\partial#1}{\partial#2}}
\newcommand\ppfrac[3]{\pfrac{^2#1}{#2\partial#3}}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\providecommand\tpa[1][0]{^{\tadj{#1}\tpchar}}% Conflict with siamltex.
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac[2]{\tfrac{\partial#1}{\partial#2}}
\newcommand\tppfrac[3]{\tpfrac{^2#1}{#2\partial#3}}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
\newcommand\Hline{\hline\Strut}

\newcommand\optsb[1]{\ifgiven{#1}{_{#1}}{}}
\newcommand\optsp[1]{\ifgiven{#1}{^{#1}}{}}
\newcommand\optindex[1]{\ifgiven{#1}{,#1}{}}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}


==> math-symbols.tex <==
% Math symbols -- requires amsmath

% Redefine some macros in math mode. Keep text mode definitions.
\let\TeXbar\_   % underscore -> \bar
\let\TeXhat\^   % undefined  -> \hat
\let\TeXtilde\~ % undefined  -> \tilde
\let\TeXcolon\: % \tmspace+\medmuskip{.2222em} -> \colon
\makeatletter
\newcommand\mcs@cc[3]{\leavevmode\ifmmode#1{#3}\else#2{#3}\fi}
\renewcommand\_{\mcs@cc\bar\TeXbar}
\renewcommand\^{\mcs@cc\hat\TeXhat}
\renewcommand\~{\mcs@cc\tilde\TeXtilde}
\renewcommand\:{\mcs@cc\colon\TeXcolon\relax}
\makeatother
\PackageInfo{math-symbols}{Redefining
 \string\_, \string\^, \string\~, \string\: in math mode.
 \MessageBreak Keeping text mode definitions.
 \MessageBreak Saving original commands as \string\TeXbar, \string\TeXhat,
 \MessageBreak \string\TeXtilde, \string\TeXcolon}

\newcommand\0\emptyset
\newcommand\bigM{M}
\newcommand\bigO{O}
\newcommand\smallo{o}
\newcommand\oo\infty
\newcommand\ox\otimes
\newcommand\x\times

\newcommand\itxt{\textup}% text in math indices
\newcommand\tsb[1]{_{\itxt{#1}}}% text subindex
\newcommand\tsp[1]{^{\itxt{#1}}}% text superindex

\newcommand\boundary\partial
\newcommand\cond\kappa
\newcommand\condabs{\cond\tsb{abs}}\newcommand\abscond\condabs
\newcommand\condrel{\cond\tsb{rel}}\newcommand\relcond\condrel
\newcommand\convrad\rho
\newcommand\eps\epsilon
\newcommand\veps\varepsilon
\newcommand\epsM{\veps\tsb{M}}
\let\epsmach\epsM
\newcommand\specrad\rho
\newcommand\spectrum\sigma
\newcommand\uvec{\mathbf1}

% Some arrows.
\newcommand\larrow\leftarrow
\newcommand\rarrow\to% \rightarrow
\newcommand\swap\leftrightarrow
\newcommand\lrarrow\swap
\newcommand\Larrow\longleftarrow
\newcommand\Rarrow\longrightarrow
\newcommand\LRarrow\longleftrightarrow
\newcommand\xlarrow\xleftarrow
\newcommand\xrarrow\xrightarrow
\newcommand\lArrow\Leftarrow
\newcommand\rArrow\Rightarrow

% Right-shifted relation symbols for alignment with :=
\newcommand\crel[1]{\mathrel{\hphantom:{#1}}}
\newcommand\isom{\crel\cong}
\newcommand\eqls{\crel=}


==> matrix.tex <==
% Matrices and column vectors -- requires amsmath

% Default space between array and delimiters.
\newcommand\matmargin{\,}
\newcommand\colmargin{\,}

% Separation lines.
\providecommand\vsl{|}
\providecommand\hsl{\hline}

% General delimited arrays: choose margin, format, delimiters.
% \Xmat{margin}{format}{ldelim}{rdelim}{entries}
\newcommand\Xmat[5][\matmargin]{%
  \left#3\begin{array}{@{#1}#2@{#1}}#5\end{array}\right#4}

% General matrices and vectors: choose margin, alignment, delimiters, ncol.
% ('<', '>' stand for ldelim, rdelim; last two args processed by \Xmat.)
% \xddmat[margin]{alignment}<nc1 nc2 nc3>{entries} (cols separated by |)
% \xdmat[margin]{alignment}<ncol1 ncol2>{entries} (cols separated by |)
% \xmat[margin]{alignment}<ncol>{entries}
% \xcol{margin}(alignment){entries}
\newcommand\xddmat[6][\matmargin]{
  \Xmat[#1]{*{#4}{#2}|*{#5}{#2}|*{#6}{#2}}{#3}}
% \Xmat[#1]{*{#4}{#2}\vsl*{#5}{#2}\vsl*{#6}{#2}}{#3}}
\newcommand\xdmat[5][\matmargin]{\Xmat[#1]{*{#4}{#2}|*{#5}{#2}}{#3}}
%\newcommand\xdmat[5][\matmargin]{\Xmat[#1]{*{#4}{#2}\vsl*{#5}{#2}}{#3}}
\newcommand\xmat[4][\matmargin]{\Xmat[#1]{*{#4}{#2}}{#3}}
\newcommand\xcol[3]{\Xmat[#1]{#3}{#2}}

% Standard matrices and vectors: choose alignment, delimiters, ncol.
\newcommand\lddmat{\xddmat[\matmargin]{l}}% \ldmat<nc1 nc2 nc3>{entries}
\newcommand\cddmat{\xddmat[\matmargin]{c}}% \cdmat<nc1 nc2 nc3>{entries}
\newcommand\rddmat{\xddmat[\matmargin]{r}}% \rdmat<nc1 nc2 nc3>{entries}
\newcommand\ddmat{\cddmat}
\newcommand\ldmat{\xdmat[\matmargin]{l}}% \ldmat<ncol1 ncol2>{entries}
\newcommand\cdmat{\xdmat[\matmargin]{c}}% \cdmat<ncol1 ncol2>{entries}
\newcommand\rdmat{\xdmat[\matmargin]{r}}% \rdmat<ncol1 ncol2>{entries}
\newcommand\dmat{\cdmat}
\newcommand\lmat{\xmat[\matmargin]{l}}% \lmat<ncol>{entries}
\newcommand\cmat{\xmat[\matmargin]{c}}% \cmat<ncol>{entries}
\newcommand\rmat{\xmat[\matmargin]{r}}% \rmat<ncol>{entries}
\newcommand\mat{\cmat}
\newcommand\col{\xcol{\colmargin}}% \col<alignment>{entries}

